EVALALIGN: Supervised Fine-Tuning Multimodal LLMs with Human-Aligned Data for Evaluating Text-to-Image Models

The recent advancements in text-to-image generative models have been remarkable. Yet, the field suffers from a lack of evaluation metrics that accurately reflect the performance of these models, particularly lacking fine-grained metrics that can guide the optimization of the models. In this paper, we propose EvalAlign, a metric characterized by its accuracy, stability, and fine granularity. Our approach leverages the capabilities of Multimodal Large Language Models (MLLMs) pre-trained on extensive data. We develop evaluation protocols that focus on two key dimensions: image faithfulness and text-image alignment. Each protocol comprises a set of detailed, fine-grained instructions linked to specific scoring options, enabling precise manual scoring of the generated images. We supervised fine-tune (SFT) the MLLM to align with human evaluative judgments, resulting in a robust evaluation model. Our evaluation across 24 text-to-image generation models demonstrate that EvalAlign not only provides superior metric stability but also aligns more closely with human preferences than existing metrics, confirming its effectiveness and utility in model assessment.

==> table/human_alignment_detail_v2.tex <==
\begin{table}
        \addtolength{\leftskip} {-0.7cm} 
	\begin{minipage}[t]{.53\textwidth}
	\centering
        \small
        \tabcolsep 2pt
        \centering
        \caption{\small \textbf{Results on image faithfulness.}} \label{tab:main_faithfulness}
            \begin{tabular}{lcc}
                \toprule
                Model & Human~~~~ & \ourmethod~~  \\
                \midrule
                PixArt XL2 1024 MS~\citep{chen2023pixart}                       & \colorbox{orange!100}{2.2848}$^{1~~}$  & \colorbox{orange!100}{1.6415}$^{1~~}$\\
                Dreamlike Photoreal v2.0~\citep{dreamlike-photoreal-20}         & \colorbox{orange!96}{2.0070}$^{2~~}$  & \colorbox{orange!88}{1.4522}$^{4~~}$  \\
                SDXL Refiner v1.0~\citep{sdxlrefiner}                           & \colorbox{orange!92}{1.9229}$^{3~~}$  & \colorbox{orange!96}{1.6072}$^{2~~}$  \\
                SDXL v1.0~\citep{sdxl}                                          & \colorbox{orange!88}{1.8136}$^{4~~}$  & \colorbox{orange!92}{1.4675}$^{3~~}$ \\
                Wuerstchen~\citep{pernias2023wuerstchen}                        & \colorbox{orange!84}{1.7837}$^{5~~}$  & \colorbox{orange!84}{1.4279}$^{5~~}$  \\
                LCM SDXL~\citep{luo2023lcm}                                     & \colorbox{orange!80}{1.6910}$^{6~~}$  & \colorbox{orange!76}{1.3391}$^{7~~}$  \\
                Openjourney~\citep{openjourne}                                  & \colorbox{orange!76}{1.6667}$^{7~~}$   & \colorbox{orange!64}{1.1750}$^{10}$  \\
                Safe SD MAX~\citep{SafeLatentDiffusion}                         & \colorbox{orange!72}{1.6491}$^{8~~}$  & \colorbox{orange!72}{1.2175}$^{8~~}$ \\
                LCM LORA SDXL~\citep{luo2023lcm}                                & \colorbox{orange!68}{1.6387}$^{9~~}$  & \colorbox{orange!80}{1.3833}$^{6~~}$ \\
                Safe SD STRONG~\citep{SafeLatentDiffusion}                     & \colorbox{orange!64}{1.6308}$^{10}$  & \colorbox{orange!60}{1.1466}$^{11}$  \\
                Safe SD MEDIUM~\citep{SafeLatentDiffusion}                     & \colorbox{orange!60}{1.6275}$^{11}$  & \colorbox{orange!44}{1.1298}$^{15}$   \\
                Safe SD WEAK~\citep{SafeLatentDiffusion}                        & \colorbox{orange!56}{1.6078}$^{12}$  & \colorbox{orange!36}{1.1188}$^{17}$ \\
                SD v2.1~\citep{Rombach_2022_sd15_sd21}                          & \colorbox{orange!52}{1.5524}$^{13}$  & \colorbox{orange!32}{1.1094}$^{18}$   \\
                SD v2.0~\citep{Rombach_2022_sd15_sd21}                         & \colorbox{orange!48}{1.5277}$^{14}$ & \colorbox{orange!48}{1.1300}$^{14}$ \\
                Openjourney v2~\citep{openjourneV2}                             & \colorbox{orange!44}{1.5000}$^{15}$  & \colorbox{orange!24}{0.9956}$^{20}$  \\
                Redshift diffusion~\citep{redshiftdiffusion}                    & \colorbox{orange!40}{1.4733}$^{16}$ &  \colorbox{orange!56}{1.1382}$^{12}$ \\
                Dreamlike Diffusion v1.0~\citep{dreamlike-diffusion-10}         & \colorbox{orange!36}{1.4652}$^{17}$  & \colorbox{orange!68}{1.2052}$^{9~~}$  \\
                SD v1.5~\citep{Rombach_2022_sd15_sd21}                          & \colorbox{orange!32}{1.4417}$^{18}$  & \colorbox{orange!52}{1.1362}$^{13}$  \\
                IF-I-XL v1.0~\citep{DeepFloydIF}                                & \colorbox{orange!28}{1.3808}$^{19}$  & \colorbox{orange!16}{0.9221}$^{22}$   \\
                SD v1.4~\citep{Rombach_2022_sd15_sd21}                          & \colorbox{orange!24}{1.3592}$^{20}$   & \colorbox{orange!20}{0.9511}$^{21}$  \\
                Vintedois Diffusion v0.1~\citep{vintedoisdiffusion}             & \colorbox{orange!20}{1.3562}$^{21}$  & \colorbox{orange!28}{1.0797}$^{19}$  \\
                IF-I-L v1.0~\citep{DeepFloydIF}                                 & \colorbox{orange!16}{1.2635}$^{22}$  & \colorbox{orange!12}{0.8814}$^{23}$  \\
                MultiFusion~\citep{MultiFusion}                                & \colorbox{orange!12}{1.2372}$^{23}$  & \colorbox{orange!40}{1.1298}$^{16}$ \\
                IF-I-M v1.0~\citep{DeepFloydIF}                                & \colorbox{orange!8}{1.0135}$^{24}$  & \colorbox{orange!8}{0.7928}$^{24}$  \\
                \bottomrule
                \end{tabular}
	\end{minipage}
        \hspace{0.28cm}
        \begin{minipage}[t]{.53\textwidth}
	\centering
        \small
        \tabcolsep 2pt
        \centering
        \caption{\small \textbf{Results on text-to-image alignment.}} \label{tab:main_t2i}
            \begin{tabular}{lcc}
                \toprule
                Model & Human~~~~ & \ourmethod~~  \\
                \midrule
                IF-I-XL v1.0~\citep{DeepFloydIF}                 & \colorbox{orange!100}{5.4500}$^{1~~}$  & \colorbox{orange!100}{5.5300}$^{1~~}$ \\
                IF-I-L v1.0~\citep{DeepFloydIF}                  & \colorbox{orange!96}{5.2300}$^{2~~}$  &\colorbox{orange!96}{5.4500}$^{2~~}$    \\
                SDXL Refiner v1.0~\citep{sdxlrefiner}            & \colorbox{orange!92}{5.2100}$^{3~~}$  & \colorbox{orange!92}{5.4000}$^{3~~}$ \\
                LCM SDXL~\citep{luo2023lcm}                      & \colorbox{orange!88}{5.1800}$^{4~~}$  & \colorbox{orange!84}{5.3300}$^{5~~}$   \\
                PixArt XL2 1024 MS~\citep{chen2023pixart}        & \colorbox{orange!84}{5.1100}$^{5~~}$  & \colorbox{orange!80}{5.3100}$^{6~~}$ \\
                IF-I-M v1.0~\citep{DeepFloydIF}                  & \colorbox{orange!80}{5.0800}$^{6~~}$  & \colorbox{orange!72}{5.2200}$^{8~~}$ \\
                LCM LORA SDXL~\citep{luo2023lcm}                 & \colorbox{orange!76}{5.0600}$^{7~~}$  & \colorbox{orange!76}{5.2700}$^{7~~}$ \\
                SDXL v1.0~\citep{sdxl}                           & \colorbox{orange!72}{5.0300}$^{8~~}$  & \colorbox{orange!88}{5.3500}$^{4~~}$ \\
                Wuerstchen~\citep{pernias2023wuerstchen}         & \colorbox{orange!68}{4.8700}$^{9~~}$  & \colorbox{orange!68}{5.1700}$^{9~~}$  \\
                Openjourney~\citep{openjourne}                   & \colorbox{orange!64}{4.8300}$^{10}$  & \colorbox{orange!46}{4.9200}$^{15}$  \\
                SD v2.1~\citep{Rombach_2022_sd15_sd21}           &  \colorbox{orange!60}{4.8000}$^{11}$    & \colorbox{orange!60}{5.0700}$^{11}$ \\
                MultiFusion~\citep{MultiFusion}                  & \colorbox{orange!56}{4.6800}$^{12}$  & \colorbox{orange!34}{4.8000}$^{18}$  \\
                Dreamlike Diffusion v1.0~\citep{dreamlike-diffusion-10}   & \colorbox{orange!54}{4.6600}$^{13}$  & \colorbox{orange!64}{5.1500}$^{10}$   \\
                SD v2.0~\citep{Rombach_2022_sd15_sd21}                    & \colorbox{orange!50}{4.6400}$^{14}$  & \colorbox{orange!56}{5.0100}$^{12}$  \\
                Vintedois Diffusion v0.1~\citep{vintedoisdiffusion}       & \colorbox{orange!46}{4.6200}$^{15}$  & \colorbox{orange!50}{4.9500}$^{14}$  \\
                Safe SD STRONG~\citep{SafeLatentDiffusion}                & \colorbox{orange!42}{4.6000}$^{16}$  & \colorbox{orange!38}{4.8300}$^{17}$  \\
                Dreamlike Photoreal v2.0~\citep{dreamlike-photoreal-20}   & \colorbox{orange!38}{4.5600}$^{17}$  & \colorbox{orange!54}{4.9800}$^{13}$ \\
                Safe SD WEAK~\citep{SafeLatentDiffusion}                  & \colorbox{orange!34}{4.5300}$^{18}$  & \colorbox{orange!26}{4.7100}$^{20}$  \\
                SD v1.4~\citep{Rombach_2022_sd15_sd21}                    & \colorbox{orange!30}{4.5200}$^{19}$  & \colorbox{orange!30}{4.7600}$^{19}$  \\
                SD v1.5~\citep{Rombach_2022_sd15_sd21}                    & \colorbox{orange!26}{4.4500}$^{20}$  & \colorbox{orange!42}{4.9000}$^{16}$  \\
                Safe SD MEDIUM~\citep{SafeLatentDiffusion}                & \colorbox{orange!22}{4.4000}$^{21}$  & \colorbox{orange!10}{4.5600}$^{24}$  \\
                Redshift diffusion~\citep{redshiftdiffusion}              & \colorbox{orange!18}{4.3500}$^{22}$  & \colorbox{orange!22}{4.6700}$^{21}$  \\
                Safe SD MAX~\citep{SafeLatentDiffusion}                   & \colorbox{orange!14}{4.3100}$^{23}$  & \colorbox{orange!14}{4.5900}$^{23}$ \\
                Openjourney v2~\citep{openjourneV2}              & \colorbox{orange!10}{4.1500}$^{24}$  & \colorbox{orange!18}{4.6500}$^{22}$  \\
                \bottomrule
                \end{tabular}
	\end{minipage}
\end{table}


